Local Advantage Networks for Cooperative Multi-Agent Reinforcement Learning

Many recent successful off-policy multi-agent reinforcement learning (MARL) algorithms for cooperative partially observable environments focus on finding factorized value functions, leading to convoluted network structures. Building on the structure of independent Q-learners, our LAN algorithm takes a radically different approach, leveraging a dueling architecture to learn for each agent a decentralized best-response policies via individual advantage functions. The learning is stabilized by a centralized critic whose primary objective is to reduce the moving target problem of the individual advantages. The critic, whose network's size is independent of the number of agents, is cast aside after learning. Evaluation on the StarCraft II multi-agent challenge benchmark shows that LAN reaches state-of-the-art performance and is highly scalable with respect to the number of agents, opening up a promising alternative direction for MARL research.

==> math_commands2.tex <==

\usepackage{amsmath,amsfonts,bm}
\usepackage{mathabx}
\usepackage{dsfont}
\usepackage{nicefrac}

\newcommand{\tabitem}{~~\llap{\textbullet}~~}
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother

\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{property}[theorem]{Property}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{notation}{Notation}
\newenvironment{proofsketch}{%
  \renewcommand{\proofname}{Proof sketch}\proof}{\endproof}


\newcommand{\tuple}[1]{\ensuremath{\left\langle #1 \right\rangle}}
\newcommand{\indexof}[2]{\ensuremath{#1_{\scriptscriptstyle #2}}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\fun}[1]{\ensuremath{\mathopen{}\mathclose\bgroup\left(#1\aftergroup\egroup\right)}}
\newcommand{\condition}[1]{\ensuremath{\1_{#1}}}
\newcommand{\diracimpulsesymbol}{\ensuremath{\delta}}
\newcommand{\diracimpulse}[2]{\ensuremath{\diracimpulsesymbol_{#2}\fun{#1}}}
\newcommand{\vect}[1]{\ensuremath{\bm{#1}}}
\newcommand{\entrywise}[3]{\ensuremath{\tuple{#1}_{#2 \in [#3]}}}
\newcommand{\images}[1]{\ensuremath{\mathrm{Im}\fun{#1}}}
\newcommand{\diam}[1]{\ensuremath{\mathrm{diam}\fun{#1}}}

\newcommand{\mdp}{\ensuremath{\mathcal{M}}}
\newcommand{\states}{\ensuremath{\mathcal{S}}}
\newcommand{\actions}{\ensuremath{\mathcal{A}}}
\newcommand{\transitions}{\ensuremath{\mathcal{T}}}
\newcommand{\probtransitions}{\ensuremath{\mathbf{P}}} %
\newcommand{\rewards}{\ensuremath{\mathcal{R}}}
\newcommand{\labels}{\ensuremath{\ell}}
\newcommand{\atomicprops}{\ensuremath{\mathbf{AP}}}
\newcommand{\sinit}{\ensuremath{s_{\mathit{I}}}}
\newcommand{\mdptuple}{\langle \states, \actions, \probtransitions, \rewards, \allowbreak \sinit, \discount \rangle}
\newcommand{\mdpspace}{\ensuremath{\mathbb{M}}}
\newcommand{\statesmdptuple}[2]{\ensuremath{ \tuple{#1, \actions, \transitions_{\scriptscriptstyle#1}, \rewards_{\scriptscriptstyle#1}, \labels_{\scriptscriptstyle#1}, \atomicprops, #2} }}
\newcommand{\previousstate}{\ensuremath{\state^{\scriptscriptstyle -1}}}
\newcommand{\previousaction}{\ensuremath{\action^{\scriptscriptstyle -1}}}
\newcommand{\state}{\ensuremath{s}}
\newcommand{\vstate}{\ensuremath{\vs}}
\newcommand{\action}{\ensuremath{a}}
\newcommand{\vaction}{\ensuremath{\va}}
\newcommand{\reward}{\ensuremath{r}}
\newcommand{\labeling}{\ensuremath{l}}
\newcommand{\labelset}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\actbot}{\ensuremath{\bot}}
\newcommand{\act}[1]{\ensuremath{\mathit{Act}\ifthenelse{\equal{#1}{}}{}{(#1)}}}
\newcommand{\trajectories}[1]{\ensuremath{\mathit{Traj}^{fin}_{ #1 }}}
\newcommand{\inftrajectories}[1]{\ensuremath{\mathit{Traj}_{#1}}}
\newcommand{\seq}[2]{\ensuremath{#1_{\scriptscriptstyle 0:#2}}}
\newcommand{\trajectory}{\tau}
\newcommand{\trajectorytuple}[3]{\ensuremath{\tuple{#1_{\scriptscriptstyle 0:#3}, #2_{\scriptscriptstyle 0: #3-1}}}}
\newcommand{\trace}{\ensuremath{\hat{\trajectory}}}
\newcommand{\tracetuple}[5]{\ensuremath{\tuple{#1_{\scriptscriptstyle 0:#5}, #2_{\scriptscriptstyle 0: #5-1}, #3_{\scriptscriptstyle 0:#5 - 1}, #4_{\scriptscriptstyle 0: #5}}}}
\newcommand{\defaulttrace}{\ensuremath{\tracetuple{\state}{\action}{\reward}{\labeling}{T}}}
\newcommand{\traces}[1]{\ensuremath{\mathit{Traces}_{#1}}}
\newcommand{\policy}{\ensuremath{\pi}}
\newcommand{\policies}[1]{\ensuremath{\Pi_{#1}}}
\newcommand{\mpolicies}[1]{\ensuremath{\Pi_{#1}}}
\newcommand{\policystates}{\ensuremath{Q}}
\newcommand{\policystate}{\ensuremath{q}}
\newcommand{\policyalphabet}{\ensuremath{\Sigma}}
\newcommand{\qinit}{\ensuremath{q_I}}
\newcommand{\mealyaction}[1]{\ensuremath{#1_{\alpha}}}
\newcommand{\mealyupdate}[1]{\ensuremath{#1_{\mu}}}
\newcommand{\mealymachine}[1]{\ensuremath{\tuple{\policystates, \mealyaction{#1}, \mealyupdate{#1}, \policystate_{I}}}}
\newcommand{\safepolicy}[1]{\ensuremath{\Pi_{#1}^{\textnormal {safe}}}}
\newcommand{\steadystate}[1]{\ensuremath{\xi_{#1}}}
\newcommand{\car}{\ensuremath{\scaleto{\rotatebox[origin=c]{90}{$\circlearrowright$}}{1.4ex}}}
\newcommand{\selfloop}[2]{\ensuremath{#1^{\nobreak\hspace{.065em} \car #2 }}}
\newcommand{\getstates}[1]{\ensuremath{\llbracket #1 \rrbracket}}
\newcommand{\valuessymbol}[2]{\ensuremath{{V}_{#1}^{#2}}}
\newcommand{\values}[3]{\ensuremath{\valuessymbol{#1}{#2}\fun{#3}}}
\newcommand{\approxvalues}[3]{\ensuremath{\hat{V}_{#1}^{#2}\fun{#3}}}
\newcommand{\episodereturn}[1]{\ensuremath{\mathbf{R}_{#1}}}
\newcommand{\qvaluessymbol}[2]{\ensuremath{Q_{#1}^{#2}}}
\newcommand{\qvalues}[4]{\ensuremath{\qvaluessymbol{#1}{#2}\fun{#3, #4}}}
\newcommand{\objective}{\ensuremath{\Omega}}
\newcommand{\bscc}[2]{\ensuremath{\mathcal{B}^{#1}_{#2}}}
\newcommand{\stationary}[1]{\ensuremath{\xi_{#1}}}
\newcommand{\resetstate}{\ensuremath{\state_{\mathsf{reset}}}}
\newcommand{\sreset}{\ensuremath{\state_{\mathsf{reset}}}}

\newcommand{\pomdp}{\ensuremath{\mathcal{P}}}
\newcommand{\observations}{\ensuremath{\Omega}}
\newcommand{\observationfn}{\ensuremath{\mathcal{O}}}
\newcommand{\observation}{\ensuremath{o}}
\newcommand{\pomdptuple}{\ensuremath{\tuple{\mdp, \observations, \observationfn}}}
\newcommand{\historytuple}[3]{\ensuremath{\tuple{#1_{\scriptscriptstyle 0:#3-1}, #2_{\scriptscriptstyle 1: #3}}}}
\newcommand{\histories}{\ensuremath{\fun{\actions \cdot \observations}^{*}}}
\newcommand{\historydistribution}{\ensuremath{\mathcal{H}}}
\newcommand{\episodes}{\ensuremath{\mathcal{E}}}
\newcommand{\history}{\ensuremath{h}}
\newcommand{\hreset}{\ensuremath{h}_{\textsf{reset}}}
\newcommand{\belief}{\ensuremath{b}}
\newcommand{\beliefs}{\ensuremath{\mathcal{B}}}
\newcommand{\beliefupdate}{\ensuremath{\tau}}
\newcommand{\beliefmdp}{\ensuremath{\mdp_{\scriptscriptstyle \beliefs}}}
\newcommand{\binit}{\ensuremath{\belief_I}}
\newcommand{\beliefprobtransitions}{\ensuremath{\probtransitions_{\scriptscriptstyle \beliefs}}}
\newcommand{\beliefrewards}{\ensuremath{\rewards_{\scriptscriptstyle \beliefs}}}
\newcommand{\beliefmdptuple}{\ensuremath{\langle\beliefs, \actions, \beliefprobtransitions, \beliefrewards, \binit,\allowbreak \discount \rangle}}
\newcommand{\augmentedpomdp}{\ensuremath{\pomdp^{\scriptscriptstyle\uparrow}}}
\newcommand{\augmentedobservationfn}{\ensuremath{\bar{\observationfn}_{\mu}}}
\newcommand{\augmentedobservationfnoriginal}{\ensuremath{\observationfn^{\scriptscriptstyle\uparrow}}}
\newcommand{\pomdpbisim}{\ensuremath{\rightrightarrows^{\scriptscriptstyle \beliefupdate}_{\scriptscriptstyle \beliefencoder}}}

\newcommand{\encodersymbol}{\embed}
\newcommand{\encoder}{\ensuremath{\encodersymbol_\encoderparameter}}
\newcommand{\encoderinit}{\ensuremath{\encodersymbol_{\encoderparameter, I}}}
\newcommand{\decodersymbol}{\ensuremath{\psi}}
\newcommand{\decoder}{\ensuremath{\decodersymbol_{\decoderparameter}}}
\newcommand{\latenttransitions}{\ensuremath{\transitions_\theta}}
 \newcommand{\encoderparameter}{\ensuremath{}}
\newcommand{\decoderparameter}{\ensuremath{}}
\newcommand{\generative}{\ensuremath{\mathcal{G}}}
\newcommand{\wassersteinparameter}{\ensuremath{\omega}}


\newcommand{\discount}{\ensuremath{\gamma}}
\newcommand{\discountedreturn}[1]{\ensuremath{\mathit{Disc}_{#1}}}
\newcommand{\totalreturn}{\ensuremath{\rewards^{\scriptscriptstyle \infty}}}
\newcommand{\unsafe}{\ensuremath{\mathit{Unsafe}}}
\newcommand{\safe}{\ensuremath{\mathit{Safe}}}
\newcommand{\always}{\ensuremath{\square}}
\newcommand{\eventually}{\ensuremath{\lozenge}}
\newcommand{\policyequiv}{\ensuremath{R}}
\newcommand{\until}[2]{\ensuremath{#1 \, \mathcal{U} \, #2}}

\newcommand{\Prob}{\ensuremath{\displaystyle \mathbb{P}}}
\newcommand{\measurableset}{\ensuremath{\mathcal{X}}}
\newcommand{\varmeasurableset}{\ensuremath{\mathcal{Y}}}
\newcommand{\borel}[1]{\ensuremath{\Sigma\fun{#1}}}
\newcommand{\sample}[2]{\ensuremath{\displaystyle #1 \sim #2}}
\newcommand{\sampledot}{\ensuremath{{\cdotp}}}
\newcommand{\expectedsymbol}[1]{\ensuremath{\mathop{\mathbb{E}}\ifthenelse{\equal{#1}{}}{}{_{#1}}}}
\newcommand{\expected}[2]{\ensuremath{\expectedsymbol{#1} \left[ #2 \right]}}
\newcommand{\expectmdp}[3]{\ensuremath{\displaystyle  \E_{#1}^{#2} [ #3 ]}}
\newcommand{\entropy}[1]{\ensuremath{\displaystyle H(#1)}}
\newcommand{\divergencesymbol}{\ensuremath{D}}
\newcommand{\divergence}[2]{\ensuremath{\divergencesymbol\fun{#1, #2}}}
\newcommand{\dklsymbol}{\ensuremath{\divergencesymbol_{{\mathrm{KL}}}}}
\newcommand{\dkl}[2]{\ensuremath{\dklsymbol\fun{#1 \parallel #2}}}
\newcommand{\dtvsymbol}{\ensuremath{d_{{TV}}}}
\newcommand{\dtv}[2]{\ensuremath{\dtvsymbol\fun{#1, #2}}}
\newcommand{\mean}{\ensuremath{\vmu}}
\newcommand{\covar}{\ensuremath{\mSigma}}
\newcommand{\normal}[3]{\ensuremath{\displaystyle \ifthenelse{\equal{#3}{}}{\mathcal{N}(#1, #2)}{\mathcal{N}(#3\,;\, #1, #2)}}}
\newcommand{\distributionssymbol}{\ensuremath{\Delta}}
\newcommand{\distributions}[1]{\ensuremath{\distributionssymbol\fun{#1}}}
\newcommand{\mode}[1]{\ensuremath{\textit{mode}\fun{#1}}}
\newcommand{\distortion}{\ensuremath{\mathbf{D}}}
\newcommand{\rate}{\ensuremath{\mathbf{R}}}
\newcommand{\dataentropy}{\ensuremath{\mathbf{H}}}
\newcommand{\elbo}{\ensuremath{\mathrm{ELBO}}}
\newcommand{\error}{\ensuremath{\varepsilon}}
\newcommand{\proberror}{\ensuremath{\delta}}

\newcommand{\logistic}[2]{\ensuremath{\mathrm{Logistic}(#1, #2)}}
\newcommand{\bernoulli}[1]{\ensuremath{\mathrm{Bernoulli}(#1)}}
\newcommand{\categorical}[1]{\ensuremath{\mathrm{Categorical}(#1)}}
\newcommand{\relaxedcategorical}[2]{\ensuremath{\mathrm{RelaxedCategorical}(#1, #2)}}
\newcommand{\relaxedbernoulli}[2]{\ensuremath{\mathrm{RelaxedBernoulli}(#1, #2)}}
\newcommand{\logit}{\ensuremath{{\alpha}}}
\newcommand{\logits}{\ensuremath{\vect{\logit}}}
\newcommand{\temperature}{\ensuremath{\lambda}}

\newcommand{\wassersteinsymbol}[1]{\ensuremath{\mathcal{W}}_{#1}}
\newcommand{\wassersteindist}[3]{\ensuremath{\wassersteinsymbol{#1}\left( #2, #3 \right)}}
\newcommand{\distance}{\ensuremath{d}}
\newcommand{\latentdistance}{\ensuremath{\bar{\distance}}}
\newcommand{\logic}{\ensuremath{\mathcal{L}}}
\newcommand{\tightoverset}[2]{%
  \tikz[baseline=(X.base),inner sep=0pt,outer sep=0pt]{%
    \node[inner sep=0pt,outer sep=0pt] (X) {$#2$}; 
    \node[yshift=1.2pt] at (X.north) {$#1$};
}}
\newcommand{\bidistance}{\ensuremath{\tightoverset{\,\scriptstyle\sim}{\distance}}}
\newcommand{\logicbidistance}{\ensuremath{\tilde{\distance}^{\logic}}}
\newcommand{\functionalexpr}{\ensuremath{\mathcal{F}_{\discount}^{\logic}}}
\newcommand{\couplings}[2]{\ensuremath{\Lambda(#1, #2)}}
\newcommand{\coupling}{\ensuremath{\lambda}}
\newcommand{\proj}{\ensuremath{\Pi}}
\newcommand{\Lipschf}[1]{\ensuremath{\mathcal{F}_{#1}}}
\newcommand{\tracedistance}{\transitiondistance}
\newcommand{\transitiondistance}{\ensuremath{\ensuremath{\vec{\distance}}}}
\newcommand{\waemdp}{W$^2\!$AE-MDP$\,$}
\newcommand{\waemdps}{W$^2\!$AE-MDPs$\,$}
\newcommand{\ncritic}{\ensuremath{n_{\scriptscriptstyle \mathcal{W}}}}

\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\overbarit}[1]{\,\overline{\!{#1}}}
\newcommand{\embed}{\ensuremath{\phi}}
\newcommand{\embeda}{\ensuremath{\psi}}
\newcommand{\actionencoder}{\ensuremath{\embed_{\encoderparameter}^{\scriptscriptstyle\actions}}}
\newcommand{\transitionencoder}{\ensuremath{\vec{\embed}}}
\newcommand{\latentmdp}{\ensuremath{\overbarit{\mdp}}}
\newcommand{\latentprobtransitions}{\ensuremath{\overbar{\probtransitions}}}
\newcommand{\latentstates}{\ensuremath{\overbarit{\mathcal{\states}}}}
\newcommand{\latentrewards}{\ensuremath{\overbarit{\rewards}}}
\newcommand{\latentlabels}{\ensuremath{\overbarit{\labels}}}
\newcommand{\latentmdptuple}{\ensuremath{\langle{\latentstates, \actions, \latentprobtransitions, \latentrewards, \zinit, \discount \rangle}}}
\newcommand{\latentobservationfn}{\ensuremath{\overbar{\observationfn}}}
\newcommand{\latentobservation}{\latentobservationfn}
\newcommand{\latentstate}{\ensuremath{\overbarit{\state}}}
\newcommand{\zinit}{\ensuremath{\latentstate_I}}
\newcommand{\latentactions}{\ensuremath{\overbarit{\actions}}}
\newcommand{\latentaction}{\ensuremath{\overbarit{\action}}}
\newcommand{\latentvaluessymbol}[2]{\overbar{\ensuremath{{V}}}_{#1}^{#2}}
\newcommand{\latentvalues}[3]{\ensuremath{\latentvaluessymbol{#1}{#2}\fun{#3}}}
\newcommand{\latentqvaluessymbol}[2]{\ensuremath{\overbarit{Q}_{#1}^{#2}}}
\newcommand{\latentqvalues}[4]{\ensuremath{\latentqvaluessymbol{#1}{#2}\fun{#3, #4}}}
\newcommand{\latentpolicy}{\ensuremath{\overbar{\policy}}}
\newcommand{\latentpolicies}{\ensuremath{\overbar{\Pi}}}
\newcommand{\latentmpolicies}{\ensuremath{\overbar{\Pi}^{\textnormal {ml}}}}
\newcommand{\latentbeliefupdate}{\ensuremath{\overbar{\tau}}}
\newcommand{\latentbelief}{\ensuremath{\overbar{\belief}}}
\newcommand{\latentbeliefs}{\ensuremath{\overbar{\beliefs}}}
\newcommand{\latentpomdp}{\ensuremath{\overbar{\pomdp}}}
\newcommand{\beliefencoder}{\ensuremath{\varphi_{\encoderparameter}}}
\newcommand{\localtransitionloss}[1]{L_{\probtransitions}}
\newcommand{\localrewardloss}[1]{L_{\rewards}}
\newcommand{\observationloss}[1]{\ensuremath{L_{\observationfn}}}
\newcommand{\beliefloss}[1]{\ensuremath{L_{\latentbeliefupdate}}}
\newcommand{\onpolicyrewardloss}[1]{\ensuremath{L_{\latentrewards}^{\varphi}}}
\newcommand{\onpolicytransitionloss}[1]{\ensuremath{L_{\latentprobtransitions}^{\varphi}}}
\newcommand{\KV}{\ensuremath{K_{\latentvaluessymbol{}{}}}}
\newcommand{\KR}[1]{\ensuremath{\ifthenelse{\equal{#1}{}}{K_{\latentrewards}}{K_{\latentrewards}^{#1}}}}
\newcommand{\KP}[1]{\ensuremath{\ifthenelse{\equal{#1}{}}{K_{\latentprobtransitions}}{K_{\latentprobtransitions}^{#1}}}}
\newcommand{\Rmax}{\ensuremath{\latentrewards^{\star}}}
\newcommand{\stationarydecoder}{{\stationary{\decoderparameter}}}
\newcommand{\latentstationaryprior}{{\bar{\xi}_{\latentpolicy_{\decoderparameter}}}}
\newcommand{\norm}[1]{\ensuremath{\left\| #1 \right\|}}
\newcommand{\gradient}{\ensuremath{\nabla}}
\newcommand{\latentvariables}{\ensuremath{\mathcal{Z}}}
\newcommand{\latentvariable}{\ensuremath{z}}
\newcommand{\originaltolatentstationary}[1]{{\latentprobtransitions_{\embed_{\encoderparameter}\stationary{\ifthenelse{\equal{#1}{}}{\policy}{#1}}}}}
\newcommand{\varsampledfrom}[3]{\ensuremath{#1}_{{#2}, {#3}}}
\newcommand{\steadystateregularizer}[1]{\ensuremath{\mathcal{W}_{\stationary{#1}}}}

\newcommand{\replaybuffer}{\ensuremath{\mathcal{D}}}
\newcommand{\experience}{\ensuremath{\eta}}
\newcommand{\loss}{\ensuremath{L}}

\newcommand{\newterm}[1]{{\bf #1}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\abs}[1]{\ensuremath{\left| #1 \right|}}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

